Simplex Autoencoders

Synthetic data generation is increasingly important due to privacy concerns. While Autoencoder-based approaches have been widely used for this purpose, sampling from their latent spaces can be challenging. Mixture models are currently the most efficient way to sample from these spaces. In this work, we propose a new approach that models the latent space of an Autoencoder as a simplex, allowing for a novel heuristic for determining the number of components in the mixture model. This heuristic is independent of the number of classes and produces comparable results. We also introduce a sampling method based on probability mass functions, taking advantage of the compactness of the latent space. We evaluate our approaches on a synthetic dataset and demonstrate their performance on three benchmark datasets: MNIST, CIFAR-10, and Celeba. Our approach achieves an image generation FID of 4.29, 13.55, and 11.90 on the MNIST, CIFAR-10, and Celeba datasets, respectively. The best AE FID results to date on those datasets are respectively 6.3, 85.3 and 35.6 we hence substantially improve those figures (the lower is the FID the better). However, AEs are not the best performing algorithms on the concerned datasets and all FID records are currently held by GANs. While we do not perform better than GANs on CIFAR and Celeba we do manage to squeeze-out a non-negligible improvement (of 0.21) over the current GAN-held record for the MNIST dataset.

==> files/blind_deconv.tex <==

\section{Improving image sharpness}
\textcolor{blue}{Not finished work}
\subsection{Blind deconvolution}
Blind deconvolution is a method used in image processing and computer vision to restore images that have been degraded by a known or unknown blur kernel. It involves estimating the blur kernel and using it to deblur the image. Blind deconvolution algorithms are useful in situations where the blur kernel is not known beforehand, or when the kernel is time-varying, such as in video deblurring. These algorithms can be applied to a variety of image types, including natural images, medical images, and satellite images. They have the potential to improve image quality, enhance image details, and remove distortions caused by blur.

One of the most well-known methods for performing blind deconvolution is the Richardson-Lucy (RL) algorithm \cite{rich}. RL is an iterative algorithm used to restore images that have been degraded by a convolutional process. It is often used to remove blur from images or to restore images that have been degraded by noise or other imperfections. This iterative method is based on the maximum likelihood principle and has been widely used in a variety of applications, including astronomy, microscopy, and medical imaging. The RL algorithm has been shown to be effective in deblurring images that have been degraded by linear shift-invariant blur kernels. However, it can struggle to deblur images that have been severely degraded or that have non-linear blur kernels. Despite these limitations, the RL algorithm remains a popular choice for blind deconvolution due to its simplicity and good performance in many cases.

The algorithm works by iteratively updating an estimate of the original image by comparing the degraded image to a convolutional model of the degradation process. At each iteration, the algorithm adjusts the estimated image to better match the degradation model, and the result is an increasingly accurate estimate of the original image.

The algorithm can be described formally as follows:

\noindent Initialize an estimate of the original image, typically with zeros or a guess at the original image.
At each iteration, perform the following steps:
\begin{enumerate}
    \item Convolve the current estimate of the original image with a model of the degradation process to produce a prediction of the degraded image.
    \item Calculate the ratio of the observed degraded image to the predicted degraded image.
    \item Convolve this ratio with the transpose of the degradation model to produce an update to the estimate of the original image.
    \item Apply this update to the current estimate of the original image.
    \item Repeat the above steps until the algorithm has converged or a maximum number of iterations has been reached.
\end{enumerate}

The algorithm can be modified by using a regularization term to prevent overfitting and by using different stopping criteria. It can also be extended to handle more complex degradation models.

\subsection{Experiments}
As noted in Goodfellow et al. (2016), using the $\ell_2$ norm to measure the quality of reconstructed input images during training often leads to blurry results. Therefore, applying blind deconvolution can improve the sharpness and overall quality of the output. The use of blind deconvolution significantly improves the output as measured by the Fréchet Inception Distance (FID) metric. Table \ref{tab:blind_deconv_fid} presents the FID scores for raw and deconvolved outputs, and Figure \ref{fig:blind_deconv_sample_img} illustrates the visual impact of blind deconvolution on three datasets.

Blind deconvolution was performed using the RL algorithm implemented in the Scikit-image library\footnote{\texttt{restoration.richardson\_lucy} function of \cite{scikit-image}.}. An initial Point Spread Function (PSF) was set as a $3\times 3$ matrix filled with the value $1/9$. The RL algorithm was run for thirty iterations, and the blind deconvolution was applied to each channel separately.

\begin{table}[H]
    \centering
    \begin{tabular}{|cc|c|c|c|}\toprule
        ~~ ~~ &                            &~~\textbf{MNIST}~~&~~\textbf{CIFAR-10}~~&~~\textbf{Celeba}~~\\\midrule
        FID   &~(no RL deconvolution)      & 4.29             & 13.55 & -  \\
        FID   &~(after RL deconvolution)   & 9.14             & 18.85 & - \\\bottomrule
    \end{tabular}
    \caption{The experimental effect of RL deconvolution on the FID.}
    \label{tab:blind_deconv_fid}
\end{table}

\begin{figure}[H]
    \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/MNIST/blind_deconv_mnist.eps}
         \caption{Visual illustration of RL's effect on the MNIST dataset.}
     \end{subfigure}
     \hfill
     \begin{subfigure}{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/CIFAR-10/cifar_samples_blind_deconv.eps}
         \caption{Visual illustration of RL's effect on the CIFAR-10 dataset.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Celeba/face_samples_blind_deconv_.eps}
         \caption{Visual illustration of RL's effect on the Celeba dataset.}
     \end{subfigure}

    \caption{Synthetic images sampled from the latent space of Simplex AE before and after blind deconvolution using the RL algorithm. For each dataset, the first line represents the initial images and the second line represents the same images after applying the RL algorithm.}
    \label{fig:blind_deconv_sample_img}
\end{figure}


==> files/preambule.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}  % pour prendre en consideration les accents
\usepackage[english]{babel}
\usepackage{hyperref, url, amsmath, amssymb}
\usepackage[ruled]{algorithm2e}
\usepackage{authblk}
\usepackage[margin=2cm]{geometry}

%\usepackage[utf8]{inputenc}
%usepackage[T1]{fontenc}
\usepackage{booktabs}
\usepackage{lscape}
\usepackage{cite}
\usepackage{mathtools,amssymb,amsmath}
\usepackage{enumerate}
\usepackage{varioref}
\usepackage{amsmath,mathpazo}
%\usepackage[pdfpagelabels=true]{hyperref}
\usepackage{cleveref}
\usepackage{xcolor}
\usepackage{algpseudocode}
%\usepackage{algorithm}
\usepackage{listings}
\usepackage{csquotes}
\usepackage{url}
\usepackage{subcaption}
\usepackage{multirow}
\usepackage{float}

\newcommand{\dir}{\mbox{Dir}}
\newcommand{\ddim}{\mbox{dim}}
\newcommand{\conv}{\mbox{Conv}}
\newcommand{\convT}{\mbox{ConvT}}
\newcommand{\lin}{\mbox{Linear}}
\newcommand{\resh}{\mbox{Reshape}}
\newcommand{\comp}{\mbox{{\scriptsize comp}}}
\newcommand{\best}{\mbox{{\scriptsize best}}}
% Keywords command
\providecommand{\keywords}[1]
{
  \small	
  \textbf{\textit{Keywords---}} #1
}
